How Do LLMs See Charts? A Comparative Study on High-Level Visualization Comprehension in Humans and LLMs

Designers often create visualizations to achieve specific high-level analytical or communication goals. These goals require people to extract complex and interconnected data patterns. Prior perceptual studies of visualization effectiveness have focused on low-level tasks, such as estimating statistical quantities, and have recently explored high-level comprehension of visualization. Despite the growing use of Large Language Models (LLMs) as visualization interpreters, how their interpretations relate to human understanding or what reasoning processes underlie their responses remains insufficiently understood. In this work, we explore LLMs' visualization comprehension, examining the alignment between designers' communicative goals and what their audience sees in a visualization. We have conducted a qualitative study to investigate the gap between human interpretative strategies and the reasoning pathways of LLMs across three types of visualizations, line graphs, bar graphs, and scatterplots, to identify the high-level patterns generated by LLMs using three prompt conditions. Our analysis results indicate that LLMs exhibit a consistent interpretative strategy that remains unchanged across prompt constraints. Furthermore, we observe two distinct approaches: humans naturally synthesize data into trend-centric narratives, whereas LLMs persist with a structural enumeration of comparisons and numerical ranges. Lastly, we see LLMs achieve visualization comprehension through mechanisms distinct from human intuition, pointing to critical challenges and new opportunities for visualization design.

==> Table/sup1_statistical_task_model_chart_type_.tex <==
\begin{table}[t]
\centering
\caption{Average count of statistical tasks performed by each LLM across different chart types under three prompt constraints.}
\label{tab:supp_charttype_tasks}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc|ccc} % 첫 번째 컬럼 l -> c 변경
\toprule
% 첫 번째 행: 모델명 (3칸씩 병합)
\multirow{2}{*}{\textbf{Chart Type}} & \multicolumn{3}{c|}{\textbf{GPT-4o}} & \multicolumn{3}{c|}{\textbf{Gemini-2.5-Flash}} & \multicolumn{3}{c}{\textbf{Claude-Sonnet-4}} \\ \cmidrule{2-10}
% 두 번째 행: 세부 조건 (PC0, PC1, PC2)
 & PC0 & PC1 & PC2 & PC0 & PC1 & PC2 & PC0 & PC1 & PC2 \\ \midrule
Bar Chart & 3.55 & 2.90 & 2.45 & 4.95 & 2.70 & 2.10 & 4.55 & 3.25 & 3.05 \\ \midrule
Line Chart & 4.15 & \textbf{3.45} & \textbf{2.70} & 5.45 & \textbf{3.15} & \textbf{2.45} & \textbf{5.40} & \textbf{4.10} & \textbf{3.55} \\ \midrule
Scatter Plot & \textbf{4.45} & 3.20 & 2.25 & \textbf{5.90} & 3.10 & 2.15 & 5.10 & 3.40 & 2.95 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> Table/sup2_statistical_task_model_sub_type_.tex <==
\begin{table}[t]
\centering
\caption{Average count of statistical tasks performed by each LLM across different data and composition types (SC: Single Class, MC: Multi Class, J: Juxtaposed) under three prompt constraints.}
\label{tab:supp_datatype_tasks}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{c|ccc|ccc|ccc} % 첫 번째 컬럼 l -> c 변경
\toprule
\multirow{2}{*}{\textbf{Composition Type}} & \multicolumn{3}{c|}{\textbf{GPT-4o}} & \multicolumn{3}{c|}{\textbf{Gemini-2.5-Flash}} & \multicolumn{3}{c}{\textbf{Claude-Sonnet-4}} \\ 
\cmidrule{2-10} 
 & PC0 & PC1 & PC2 & PC0 & PC1 & PC2 & PC0 & PC1 & PC2 \\ \midrule
SC  & 3.66 & 3.06 & 2.26 & 5.06 & 3.13 & \textbf{2.40} & 5.13 & 3.66 & 3.06 \\ \midrule
MC   & 4.06 & 3.20 & 2.26 & \textbf{5.66} & \textbf{3.40} & 2.33 & 5.06 & \textbf{3.80} & \textbf{3.53} \\ \midrule
SC-J & \textbf{4.53} & \textbf{3.40} & \textbf{2.73} & \textbf{5.66} & 2.86 & 2.26 & \textbf{5.26} & 3.53 & 2.93 \\ \midrule
MC-J & 3.93 & 3.06 & 2.60 & 5.33 & 2.53 & 1.93 & 4.60 & 3.33 & 3.20 \\ \bottomrule
\end{tabular}
}
\end{table}

==> Table/taxonomy_table.tex <==
\begin{table*}[h!]
\centering
\caption{HLC Task Classification based on Bloom's Taxonomy}
\label{tab:blooms_mapping_final}
% To make the table fit within the text width, we use \resizebox
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}llll@{}}
\toprule
\textbf{Level} & \textbf{Bloom's Level} & \textbf{Semantic Content (Task Definition)} & \textbf{Mapped HLC Tasks} \\ \midrule
\textbf{1} & \textbf{Remember} & Recalling explicit, single facts or values from the chart. & \begin{tabular}[t]{@{}l@{}}\texttt{Extremum}, \texttt{Determine Range}\end{tabular} \\ \addlinespace
\textbf{2} & \textbf{Understand} & Describing or summarizing relationships between two or more data points. & \begin{tabular}[t]{@{}l@{}}\texttt{Comparison}\end{tabular} \\ \addlinespace
\textbf{3} & \textbf{Apply} & Using a known procedure (calculation) to derive new values from the data. & \begin{tabular}[t]{@{}l@{}}\texttt{Compute Derived Value},\\ \texttt{Characterize Distribution}  \end{tabular} \\ \addlinespace
\textbf{4} & \textbf{Analyze} & Inferring hidden patterns, structures, or relationships across the entire dataset. & \begin{tabular}[t]{@{}l@{}}\texttt{Anomaly}, \texttt{Correlation}, \\  \texttt{Cluster}, \texttt{Trend}\end{tabular} \\ \bottomrule
\end{tabular}%
}
\end{table*}
